Multi-Agent Combinatorial Path Finding with Heterogeneous Task Duration

Multi-Agent Combinatorial Path Finding (MCPF) seeks collision-free paths for multiple agents from their initial locations to destinations, visiting a set of intermediate target locations in the middle of the paths, while minimizing the sum of arrival times. While a few approaches have been developed to handle MCPF, most of them simply direct the agent to visit the targets without considering the task duration, i.e., the amount of time needed for an agent to execute the task (such as picking an item) at a target location. MCPF is NP-hard to solve to optimality, and the inclusion of task duration further complicates the problem. This paper investigates heterogeneous task duration, where the duration can be different with respect to both the agents and targets. We develop two methods, where the first method post-processes the paths planned by any MCPF planner to include the task duration and has no solution optimality guarantee; and the second method considers task duration during planning and is able to ensure solution optimality. The numerical and simulation results show that our methods can handle up to 20 agents and 50 targets in the presence of task duration, and can execute the paths subject to robot motion disturbance.

==> source/analysis.tex <==

\subsection{Properties of \abbrCBSS}
\subsubsection{Conflict-Free}
\label{ana:conflict-free_cbssstn}
% We now prove that \abbrCBSS can guarantee 
% \begin{lemma}
% The joint path returned by \abbrTPGD is conflict-free. 
% \end{lemma}

% \begin{proof}

% \end{proof}

% \begin{theorem}
% (Small results use lemma, big results use theorem)
% \end{theorem}

% \begin{proof}

% \end{proof}

% In \abbrTPGD, given a joint path $\pi$, the task duration $\tau$ and a TPG $\mathcal{G}$, we only need to prove that the output joint path $\pi_c$ will follow the same visiting order in $\pi$ for each agent because the visiting order in $\pi$ itself is conflict-free. The visiting order in joint path can be divided into two parts:
% \begin{itemize}
%     \item For the visiting order in the single path $\pi_c^i \in \pi_c$ of each agent $i$, it follows the same as the single path $\pi^i \in \pi$. That's the Type 1 edges in $\mathcal{G}$ are constructed according to the visiting order in $\pi^i \in \pi$, and due to the condition (i) in \textit{CheckDelete} in Algorithm~\ref{alg:tpg}, any vertex $s \in \mathcal{V}$ can be deleted only if the previous vertices are deleted (i.e the in-degree of $s$ is zero). Thus, agent $i$ going along path $\pi_c^i$ will follow exactly the visiting order in $\pi^i$.
%     \item For the visiting order to the same vertex between two different agents $i$ and $j, i\neq j$, $\pi_c$ follows the same as $\pi$ because of three conditions in \textit{CheckDelete} in Algorithm~\ref{alg:tpg}. For example, agent $i$ and $j$ will visit the same location $v \in V$ at time $t$ and $t', (t'>t)$, correspongding to $s_t^i, s_{t'}^j \in \mathcal{V}$ respectively in $\pi$. But with task duration $\tau$ incorporated in $\pi_c$, agent $i$ or $j$ may be delayed due to some task execution along the joint path $\pi_c$. Thus, it may bring conflict at $v$ between agent $i$ and $j$ since they are delayed differently (e.g. agent $i$ spends additional $t'-t$ time units before visiting $s_t^i$ along $\pi_c^j$ while agent $j$ has no task to execute before visiting $s_{t'}^j$ along $\pi_c^j$). However, with the three conditions in \textit{CheckDelete}, even if there exists a conflict after considering task duration, agent $j$ and $i$ will not visit $s_{t'}^j$ and $s_t^i$ at the same time in $\pi_c$ because the conditions of deleting the Type 2 edge $(s_t^i, s_{t'}^j)$ will not be satisfied until agent $i$ finishes all the tasks before (and at) vertex $s_t^i$ and visit the next vertex.
% \end{itemize}

\subsection{Properties of \abbrCBXS}
\label{ana:cbxs}
% \subsubsection{Completeness of the Branching Rule}
% \label{ana:complete_cbxs}
% We say that two sets of constraints corresponding to agent $i$ and $j$ are \textit{mutually disjunctive}~\cite{li2019multi} iff any conflict-free joint path satisfies at least one of the two sets of constraints. Here, we can prove our branching rule always generates two \textit{mutually disjunctive} sets of constraints $C_1$ and $C_2$ from one conflict $cft$. If not, the conflict $cft$ must exist in the conflict-free joint path which is contradictory.

% Therefore, drawing on any joint sequence $\gamma$, with our proposed branching rule, we can find all the conflict-free joint path from $\gamma$ by resolve the conflicts along the $\gamma$. Otherwise, there exists one conflict-free joint path $\pi'$ which is not included in the search tree expanded from $\gamma$ indicating that $\pi'$ violates one pair of two sets of constraints. However, because all pairs of constraints we generate are \textit{mutually disjunctive}, $\pi'$ must have one $cft$, contradicting its collision-free characteristic. Thus, the new branching process of the search tree in Sec..~\ref{subsec:branchingrules} does not lose any set of conflict-free paths, and we say it is complete.

% \subsubsection{Solution Optimality}
% \label{ana:optimal_cbxs}
% The proof in \cite{ren2023cbss} and \cite{sharon2015conflict} can be adapted here to prove the optimality. According to \cite{ren2023cbss}, for a \abbrMCPF problem, if we set $\epsilon=0$, CBSS can return an optimal solution with minimal cost. That's because in the high-level search of CBSS, we always choose the tree node with minimal cost and the branching process of the node is complete as proved in Sec..~\ref{ana:complete_cbxs}, which means the chosen joint path is always a lower bound of the cost among all the conflict-free paths. Here, for a \abbrMATSPF problem, its difference from \abbrMCPF problem is to consider task duration when planning a target sequence in the K-best target sequencing process, while the rest of the part has no influence on the solution optimality. Since we have modified the transformation module and can compute the optimal TSP tour with task duration in \abbrMATSPF, similar to \abbrCBSS, our \abbrCBXS method still guarantees to compute an optimal solution.




==> source/noteToPrac.tex <==
The motivation of this paper originates from the need to find conflict-free paths for mobile robots to visit many target locations in warehouse logistics, manufacturing and surveillance.
While many planners have been developed for this purpose, few of them consider task duration:
Robots need time to execute the task at a target location and may block the passage needed by other robots.
To handle task duration, this paper develops two methods, analyzes their properties, and verify them with numerical tests.
We also provide high-fidelity simulations to showcase the usage of the planners for practitioners.

==> source/related.tex <==
% \subsection{Multi-agent Path Finding}

Many \abbrMAPF algorithms have been developed and span a spectrum from coupled~\cite{standley2010finding} to decoupled~\cite{silver2005hca}, trading off completeness and optimality for scalability.
In the middle of this spectrum lies the dynamically-coupled methods such as M*~\cite{wagner2015subdimensional} and CBS \cite{sharon2015conflict}, which begin by planning for each agent a shortest path from the start to the goal ignoring agent-agent collision and then couple agents for planning only when needed to avoid collision.
Dynamically-coupled methods are improved and extended in many ways~\cite{honig2018conflict,li2019multi,ren2021loosely,ren22mocbs_tase}.
All these \abbrMAPF planners find start-goal paths without considering any intermediate target locations.

% \subsection{Travelling Salesman Problem}


With intermediate targets, the planner needs to determine the assignment and visiting order of the targets for the agents.
For a single agent, the Traveling Salesman Problem (TSP), which seeks a shortest tour that visits all vertices in a graph, is a well-known NP-hard problem~\cite{Applegate:2007}.
The multi-agent version of TSP (denoted as mTSP) is more challenging since the vertices in the graph must be allocated to each agent in addition to finding the optimal visiting order of vertices.
To solve these problems, a variety of methods have been developed ranging from exact methods~\cite{Applegate:2007} to heuristics~\cite{lkh} and approximation algorithms~\cite{christofides1976worst}, trading off solution optimality for runtime efficiency.
This paper leverages the existing methods for TSP and adapt them to handle task duration.

% \subsection{Multi-agent Combinatorial Path Finding}
% Introduce two sub-problems in \abbrMCPF including mtsp problem and \abbrMAPF. List several methods to solve these two problems.

% Finally, introduce CBSS\cite{ren2023cbss} and its capability to solve \abbrMCPF. 

% \subsection{Post-Process for Multi-agent Combinatorial Path Finding}

% \subsection{Task Duration in Multi-agent Path Finding}

Some recent work combines \abbrMAPF with target assignment and sequencing (such as~\cite{honig2018conflict,ma2016optimal,ren2023cbss,ren2021ms,zhang2022multi,surynek2021multi,9197527}).
% \cite{honig2018conflict,ma2016optimal,nguyen2019generalized,surynek2021multi,zhang2022multi,zhong2022optimal,ren2023cbss,ren2021ms,Ma2017Lifelong,Liu2019mapd,xu2022multi,henkel2019optimal}.
Most of them either consider the visiting order only given that each agent is pre-allocated a set of targets~\cite{surynek2021multi,zhang2022multi}, or target assignment only without the need for computing visiting orders of targets~\cite{honig2018conflict,ma2016optimal}.

Finally, task duration at target locations has been considered when routing for unmanned vehicles~\cite{9551556} and planning for assembly \cite{9197527}.
When combining target sequencing with \abbrMAPF, task duration remains under-explored.


% \cite{9197527} generalizes \abbrMAPF problem with task assignment and considers duration for each task. However, it has no assignment constraints and its low level search process is not complete and thus may not be optimal.

% In addition, \cite{9812020} also focuses on a generalization of \abbrMAPF, whichi is the multi-goal task assignment and path finding (MG-TAPF) problem where each task consists of a sequence of goal locations and provide optimal and bounded-suboptimal solution. If we set the goal locations in the sequence of each task to be the same, the task can be transformed into the task with duration in \abbrMATSPF here, but still it does not consider assignment constraints.

% Furthermore, \cite{9551556} and \cite{8723305} considers \textit{heterogeneous} task duration in the target sequencing process. However, both of them can only provide a feasible solution satisfying all task assignments without optimality guaranteed and they do not consider the conflicts among multiple agents.
